Does Data Contamination Detection Work (Well) for LLMs? A Survey and Evaluation on Detection Assumptions

Large language models (LLMs) have demonstrated great performance across various benchmarks, showing potential as general-purpose task solvers. However, as LLMs are typically trained on vast amounts of data, a significant concern in their evaluation is data contamination, where overlap between training data and evaluation datasets inflates performance assessments. Multiple approaches have been developed to identify data contamination. These approaches rely on specific assumptions that may not hold universally across different settings. To bridge this gap, we systematically review 50 papers on data contamination detection, categorize the underlying assumptions, and assess whether they have been rigorously validated. We identify and analyze eight categories of assumptions and test three of them as case studies. Our case studies focus on detecting direct, instance-level data contamination, which is also referred to as Membership Inference Attacks (MIA). Our analysis reveals that MIA approaches based on these three assumptions can have similar performance to random guessing, on datasets used in LLM pretraining, suggesting that current LLMs might learn data distributions rather than memorizing individual instances. Meanwhile, MIA can easily fail when there are data distribution shifts between the seen and unseen instances.

==> archive/tables/overall_1.4b.tex <==

\begin{table*}[h]
\centering
\resizebox{0.98\textwidth}{!}{
\begin{tabular}{llccccccccccc}
\hline
\multicolumn{2}{l}{\textbf{Assumptions \& Metric}} 
& \textbf{Github}& \textbf{FreeLaw}& \textbf{ArXiv}& \textbf{\begin{tabular}[c]{@{}c@{}}PubMed-\\ Central\end{tabular}}& \textbf{\begin{tabular}[c]{@{}c@{}}Enron-\\ Emails\end{tabular}}& \textbf{\begin{tabular}[c]{@{}c@{}}PubMed-\\ Abstracts\end{tabular}}& \textbf{\begin{tabular}[c]{@{}c@{}}Open-\\ Subtitles\end{tabular}}& \textbf{\begin{tabular}[c]{@{}c@{}}OpenWeb-\\ Text2\end{tabular}}& \textbf{\begin{tabular}[c]{@{}c@{}}Youtube-\\ Subtitles\end{tabular}}& \textbf{\begin{tabular}[c]{@{}c@{}}Hacker-\\ News\end{tabular}}& \textbf{Pile-CC} \\\hline
\multirow{6}{*}{A\ref{as:prob_absolute}}  & PPL\_50&49.5&49.1&50.7&49.1&50.1&49.7&47.9&50.7&51.2&48.5&49.8\\
 & PPL\_100&50.8&49.5&51.0&50.1&51.2&48.5&47.6&49.3&50.9&47.4&50.2\\
 & PPL\_200&50.9&49.8&50.9&49.9&52.2&49.4&46.7&48.8&49.8&50.9&52.0\\
 & Min 5\% token&51.6&50.4&51.0&48.6&50.3&49.4&48.8&49.5&48.8&48.9&51.1\\
 & Min 15\% token&51.1&49.7&51.3&49.1&50.5&49.0&49.0&49.7&49.3&50.0&51.1\\
 & Min 25\% token&51.0&49.4&51.5&49.4&50.6&49.1&49.1&49.3&49.3&50.0&51.2\\
 \cline{1-2}\multirow{3}{*}{A\ref{as:exact_memorization}} & Mem 1&49.7&49.8&51.6&47.9&49.4&50.7&49.4&51.4&48.1&49.2&48.8\\
 & Mem 3&50.5&48.5&51.1&49.0&50.4&50.5&49.5&51.8&48.6&49.7&48.6\\
 & Mem 5&49.0&48.8&51.0&48.2&49.6&50.6&51.8&51.3&49.6&50.5&48.5\\
\cline{1-2} \multirow{3}{*}{A\ref{as:Generation_Variation}} & Entropy 5&51.9&49.6&51.9&49.7&50.1&48.0&48.1&50.8&48.2&49.4&51.3\\
 & Entropy 10&51.8&49.8&51.5&49.2&50.4&48.3&48.1&51.0&48.4&49.9&50.8\\
 & Entropy 25&51.9&49.8&51.1&49.5&50.9&48.5&46.9&50.8&48.3&49.7&50.8\\\hline
\multicolumn{2}{l}{\textbf{Average AUC}}& 50.8& 49.5& 51.2& 49.1& 50.5& 49.3& 48.6& 50.4& 49.2& 49.5& 50.3\\ \hline
 \hline\multirow{2}{*}{PPL} & Seen&3.6$\pm$3.8&4.4$\pm$2.4&9.8$\pm$4.6&8.1$\pm$3.5&8.5$\pm$5.9&9.6$\pm$4.3&16.0$\pm$6.9&14.2$\pm$7.4&16.3$\pm$19.2&15.3$\pm$5.7&17.1$\pm$12.5\\
 & Unseen&3.6$\pm$4.9&4.7$\pm$8.6&9.9$\pm$4.4&8.2$\pm$3.9&9.4$\pm$7.4&9.5$\pm$4.1&15.2$\pm$6.6&13.7$\pm$6.4&15.6$\pm$12.2&15.7$\pm$7.2&17.8$\pm$13.9\\

\hline
\end{tabular}
}
\caption{Average contamination detection AUC for the Pythia-1.4b model, under different PILE domains. `PPL' represents the average perplexity $\pm$ STD, where instances are truncated by the model max length of 2048 tokens.
}
\label{tab:results_1.4b}
\end{table*}


==> archive/tables/overall_12b.tex <==

\begin{table*}[h]
\centering
\resizebox{0.98\textwidth}{!}{
\begin{tabular}{llccccccccccc}
\hline
\multicolumn{2}{l}{\textbf{Assumptions \& Metric}} & \textbf{Github} & \textbf{\begin{tabular}[c]{@{}c@{}}Free-\\ Law\end{tabular}} & \textbf{ArXiv} & \textbf{\begin{tabular}[c]{@{}c@{}}PubMed\\ Central\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Enron\\ Emails\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}PubMed\\ Abstracts\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Open-\\ Subtitles\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}OpenWeb-\\ Text2\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Youtube-\\ Subtitles\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Hacker-\\ News\end{tabular}} & \textbf{Pile-CC} \\\hline
\multirow{6}{*}{A\ref{as:prob_absolute}}  & PPL\_50&49.7&48.9&50.7&49.4&49.6&49.7&47.9&50.3&50.8&48.4&49.8\\
 & PPL\_100&50.8&49.4&51.1&50.1&50.5&48.8&48.1&48.9&50.3&47.3&50.4\\
 & PPL\_200&51.1&49.4&50.9&50.2&51.4&49.9&47.8&48.5&49.5&50.7&52.1\\
 & Min 5\% token&51.5&49.8&51.3&48.5&50.0&48.5&49.8&49.7&49.0&47.8&50.9\\
 & Min 15\% token&51.2&49.8&51.3&49.2&50.1&49.4&49.9&49.2&49.2&49.6&51.1\\
 & Min 25\% token&51.0&49.4&51.4&49.5&50.0&49.6&50.2&49.0&49.2&49.8&51.1\\
 \cline{1-2}\multirow{3}{*}{A\ref{as:exact_memorization}} & Mem 1&49.2&48.9&50.5&47.1&49.8&50.7&49.6&50.6&49.4&48.3&49.7\\
 & Mem 3&49.7&50.0&51.0&46.5&50.1&49.8&51.5&50.5&48.2&49.3&48.7\\
 & Mem 5&49.7&48.0&50.8&48.2&49.7&52.7&50.8&50.2&49.1&50.0&49.4\\
\cline{1-2} \multirow{3}{*}{A\ref{as:Generation_Variation}} & Entropy 5&51.9&49.2&52.4&48.9&50.3&48.0&49.4&51.9&48.6&49.0&50.4\\
 & Entropy 10&52.2&49.4&52.3&49.3&50.4&48.2&48.7&52.1&48.6&49.0&50.6\\
 & Entropy 25&52.1&49.5&50.9&49.5&50.7&48.5&48.1&51.0&48.1&49.6&50.9\\
\hline\multirow{2}{*}{PPL} & Seen&2.8$\pm$5.4&3.8$\pm$1.3&5.4$\pm$2.6&5.4$\pm$1.9&6.8$\pm$8.9&8.2$\pm$4.0&8.6$\pm$3.5&10.0$\pm$7.9&10.3$\pm$12.6&11.1$\pm$5.3&13.1$\pm$11.1\\
 & Unseen&2.9$\pm$6.0&3.8$\pm$2.7&5.4$\pm$2.0&5.4$\pm$2.1&7.0$\pm$9.4&8.1$\pm$3.9&8.6$\pm$3.7&9.9$\pm$8.0&10.1$\pm$12.5&10.8$\pm$4.8&13.0$\pm$9.7\\

    \hline
    \end{tabular}
    }
    \caption{Average contamination detection AUC for the \textbf{Pythia-12b} model, under different PILE domains. `PPL' represents the average perplexity $\pm$ STD, where instances are truncated by the model max length of 2048 tokens.
    }
    \label{tab:results_12b}
    \end{table*}
    

==> archive/tables/overall_160m.tex <==

\begin{table*}[h]
\centering
\resizebox{0.98\textwidth}{!}{
\begin{tabular}{llccccccccccc}
\hline
\multicolumn{2}{l}{\textbf{Assumptions \& Metric}} & \textbf{Github} & \textbf{\begin{tabular}[c]{@{}c@{}}Free-\\ Law\end{tabular}} & \textbf{ArXiv} & \textbf{\begin{tabular}[c]{@{}c@{}}PubMed\\ Central\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Enron\\ Emails\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}PubMed\\ Abstracts\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Open-\\ Subtitles\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}OpenWeb-\\ Text2\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Youtube-\\ Subtitles\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Hacker-\\ News\end{tabular}} & \textbf{Pile-CC} \\\hline
\multirow{6}{*}{A\ref{as:prob_absolute}}  & PPL\_50&49.7&48.9&50.7&49.4&49.6&49.7&47.9&50.3&50.8&48.4&49.8\\
 & PPL\_100&50.8&49.4&51.1&50.1&50.5&48.8&48.1&48.9&50.3&47.3&50.4\\
 & PPL\_200&51.1&49.4&50.9&50.2&51.4&49.9&47.8&48.5&49.5&50.7&52.1\\
 & Min 5\% token&51.5&49.8&51.3&48.5&50.0&48.5&49.8&49.7&49.0&47.8&50.9\\
 & Min 15\% token&51.2&49.8&51.3&49.2&50.1&49.4&49.9&49.2&49.2&49.6&51.1\\
 & Min 25\% token&51.0&49.4&51.4&49.5&50.0&49.6&50.2&49.0&49.2&49.8&51.1\\
 \cline{1-2}\multirow{3}{*}{A\ref{as:exact_memorization}} & Mem 1&49.2&48.9&50.5&47.1&49.8&50.7&49.6&50.6&49.4&48.3&49.7\\
 & Mem 3&49.7&50.0&51.0&46.5&50.1&49.8&51.5&50.5&48.2&49.3&48.7\\
 & Mem 5&49.7&48.0&50.8&48.2&49.7&52.7&50.8&50.2&49.1&50.0&49.4\\
\cline{1-2} \multirow{3}{*}{A\ref{as:Generation_Variation}} & Entropy 5&51.9&49.2&52.4&48.9&50.3&48.0&49.4&51.9&48.6&49.0&50.4\\
 & Entropy 10&52.2&49.4&52.3&49.3&50.4&48.2&48.7&52.1&48.6&49.0&50.6\\
 & Entropy 25&52.1&49.5&50.9&49.5&50.7&48.5&48.1&51.0&48.1&49.6&50.9\\
\hline\multirow{2}{*}{PPL} & Seen&7.1$\pm$15.6&8.5$\pm$3.4&11.8$\pm$5.9&11.1$\pm$5.0&25.1$\pm$34.8&19.0$\pm$10.3&20.0$\pm$7.2&27.3$\pm$23.9&25.2$\pm$29.9&28.5$\pm$15.2&33.1$\pm$29.8\\
 & Unseen&7.4$\pm$18.8&8.9$\pm$9.7&12.1$\pm$5.1&11.0$\pm$5.0&25.5$\pm$30.8&18.8$\pm$11.3&19.9$\pm$6.4&26.9$\pm$19.3&24.8$\pm$25.2&27.9$\pm$14.2&32.9$\pm$24.3\\

    \hline
    \end{tabular}
    }
    \caption{Average contamination detection AUC for the \textbf{Pythia-160m} model, under different PILE domains. `PPL' represents the average perplexity $\pm$ STD, where instances are truncated by the model max length of 2048 tokens.
    }
    \label{tab:results_160m}
    \end{table*}
    

==> archive/tables/overall_2.8b.tex <==

\begin{table*}[h]
\centering
\resizebox{0.98\textwidth}{!}{
\begin{tabular}{llccccccccccc}
\hline
\multicolumn{2}{l}{\textbf{Assumptions \& Metric}} & \textbf{Github} & \textbf{\begin{tabular}[c]{@{}c@{}}Free-\\ Law\end{tabular}} & \textbf{ArXiv} & \textbf{\begin{tabular}[c]{@{}c@{}}PubMed\\ Central\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Enron\\ Emails\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}PubMed\\ Abstracts\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Open-\\ Subtitles\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}OpenWeb-\\ Text2\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Youtube-\\ Subtitles\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Hacker-\\ News\end{tabular}} & \textbf{Pile-CC} \\\hline
\multirow{6}{*}{A\ref{as:prob_absolute}}  & PPL\_50&49.7&48.9&50.7&49.4&49.6&49.7&47.9&50.3&50.8&48.4&49.8\\
 & PPL\_100&50.8&49.4&51.1&50.1&50.5&48.8&48.1&48.9&50.3&47.3&50.4\\
 & PPL\_200&51.1&49.4&50.9&50.2&51.4&49.9&47.8&48.5&49.5&50.7&52.1\\
 & Min 5\% token&51.5&49.8&51.3&48.5&50.0&48.5&49.8&49.7&49.0&47.8&50.9\\
 & Min 15\% token&51.2&49.8&51.3&49.2&50.1&49.4&49.9&49.2&49.2&49.6&51.1\\
 & Min 25\% token&51.0&49.4&51.4&49.5&50.0&49.6&50.2&49.0&49.2&49.8&51.1\\
 \cline{1-2}\multirow{3}{*}{A\ref{as:exact_memorization}} & Mem 1&49.2&48.9&50.5&47.1&49.8&50.7&49.6&50.6&49.4&48.3&49.7\\
 & Mem 3&49.7&50.0&51.0&46.5&50.1&49.8&51.5&50.5&48.2&49.3&48.7\\
 & Mem 5&49.7&48.0&50.8&48.2&49.7&52.7&50.8&50.2&49.1&50.0&49.4\\
\cline{1-2} \multirow{3}{*}{A\ref{as:Generation_Variation}} & Entropy 5&51.9&49.2&52.4&48.9&50.3&48.0&49.4&51.9&48.6&49.0&50.4\\
 & Entropy 10&52.2&49.4&52.3&49.3&50.4&48.2&48.7&52.1&48.6&49.0&50.6\\
 & Entropy 25&52.1&49.5&50.9&49.5&50.7&48.5&48.1&51.0&48.1&49.6&50.9\\
\hline\multirow{2}{*}{PPL} & Seen&3.3$\pm$6.6&4.2$\pm$1.5&6.1$\pm$2.8&6.0$\pm$2.2&9.4$\pm$13.3&9.3$\pm$4.8&10.8$\pm$3.2&11.9$\pm$9.4&12.1$\pm$15.3&13.1$\pm$6.6&15.4$\pm$13.8\\
 & Unseen&3.3$\pm$6.5&4.3$\pm$3.5&6.2$\pm$2.5&6.0$\pm$2.4&9.5$\pm$12.4&9.2$\pm$4.8&10.8$\pm$3.5&11.8$\pm$9.0&11.7$\pm$14.2&12.9$\pm$6.0&15.2$\pm$11.4\\

    \hline
    \end{tabular}
    }
    \caption{Average contamination detection AUC for the \textbf{Pythia-2.8b} model, under different PILE domains. `PPL' represents the average perplexity $\pm$ STD, where instances are truncated by the model max length of 2048 tokens.
    }
    \label{tab:results_2.8b}
    \end{table*}
    

==> archive/tables/overall_410m.tex <==

\begin{table*}[h]
\centering
\resizebox{0.98\textwidth}{!}{
\begin{tabular}{llccccccccccc}
\hline
\multicolumn{2}{l}{\textbf{Assumptions \& Metric}} & \textbf{Github} & \textbf{\begin{tabular}[c]{@{}c@{}}Free-\\ Law\end{tabular}} & \textbf{ArXiv} & \textbf{\begin{tabular}[c]{@{}c@{}}PubMed\\ Central\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Enron\\ Emails\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}PubMed\\ Abstracts\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Open-\\ Subtitles\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}OpenWeb-\\ Text2\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Youtube-\\ Subtitles\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Hacker-\\ News\end{tabular}} & \textbf{Pile-CC} \\\hline
\multirow{6}{*}{A\ref{as:prob_absolute}}  & PPL\_50&49.7&48.9&50.7&49.4&49.6&49.7&47.9&50.3&50.8&48.4&49.8\\
 & PPL\_100&50.8&49.4&51.1&50.1&50.5&48.8&48.1&48.9&50.3&47.3&50.4\\
 & PPL\_200&51.1&49.4&50.9&50.2&51.4&49.9&47.8&48.5&49.5&50.7&52.1\\
 & Min 5\% token&51.5&49.8&51.3&48.5&50.0&48.5&49.8&49.7&49.0&47.8&50.9\\
 & Min 15\% token&51.2&49.8&51.3&49.2&50.1&49.4&49.9&49.2&49.2&49.6&51.1\\
 & Min 25\% token&51.0&49.4&51.4&49.5&50.0&49.6&50.2&49.0&49.2&49.8&51.1\\
 \cline{1-2}\multirow{3}{*}{A\ref{as:exact_memorization}} & Mem 1&49.2&48.9&50.5&47.1&49.8&50.7&49.6&50.6&49.4&48.3&49.7\\
 & Mem 3&49.7&50.0&51.0&46.5&50.1&49.8&51.5&50.5&48.2&49.3&48.7\\
 & Mem 5&49.7&48.0&50.8&48.2&49.7&52.7&50.8&50.2&49.1&50.0&49.4\\
\cline{1-2} \multirow{3}{*}{A\ref{as:Generation_Variation}} & Entropy 5&51.9&49.2&52.4&48.9&50.3&48.0&49.4&51.9&48.6&49.0&50.4\\
 & Entropy 10&52.2&49.4&52.3&49.3&50.4&48.2&48.7&52.1&48.6&49.0&50.6\\
 & Entropy 25&52.1&49.5&50.9&49.5&50.7&48.5&48.1&51.0&48.1&49.6&50.9\\
\hline\multirow{2}{*}{PPL} & Seen&4.8$\pm$11.4&5.9$\pm$2.2&8.3$\pm$4.7&7.9$\pm$3.3&16.1$\pm$22.9&13.0$\pm$7.0&14.9$\pm$4.0&17.7$\pm$14.4&17.0$\pm$21.4&19.5$\pm$10.8&22.4$\pm$20.7\\
 & Unseen&4.7$\pm$8.7&6.1$\pm$6.0&8.5$\pm$3.6&7.9$\pm$3.4&16.2$\pm$19.5&12.9$\pm$7.3&14.9$\pm$4.5&17.5$\pm$13.4&16.6$\pm$18.4&19.2$\pm$10.3&22.3$\pm$17.3\\

    \hline
    \end{tabular}
    }
    \caption{Average contamination detection AUC for the \textbf{Pythia-410m} model, under different PILE domains. `PPL' represents the average perplexity $\pm$ STD, where instances are truncated by the model max length of 2048 tokens.
    }
    \label{tab:results_410m}
    \end{table*}
    

==> archive/tables/overall_6.9b.tex <==

\begin{table*}[h]
\centering
\resizebox{0.98\textwidth}{!}{
\begin{tabular}{llccccccccccc}
\hline
\multicolumn{2}{l}{\textbf{Assumptions \& Metric}} & \textbf{\begin{tabular}[c]{@{}c@{}}Github\\(GH)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Free-\\ Law \\ (FL)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}ArXiv\\(AX) \end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}PubMed\\ Central \\ (PC)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Enron\\ Emails \\ (EE)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}PubMed\\ Abstracts \\ (PA)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Open-\\ Subtitles \\ (OS)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}OpenWeb-\\ Text2 \\(OWT)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Youtube-\\ Subtitles \\(YS)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Hacker-\\ News \\ (HN)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Pile-CC \\ (PC)\end{tabular}}  \\\hline
\multirow{6}{*}{A\ref{as:prob_absolute}}  & PPL\_50&49.7&48.9&50.7&49.4&49.6&49.7&47.9&50.3&50.8&48.4&49.8\\
 & PPL\_100&50.8&49.4&51.1&50.1&50.5&48.8&48.1&48.9&50.3&47.3&50.4\\
 & PPL\_200&51.1&49.4&50.9&50.2&51.4&49.9&47.8&48.5&49.5&50.7&52.1\\
 & Min 5\% token&51.5&49.8&51.3&48.5&50.0&48.5&49.8&49.7&49.0&47.8&50.9\\
 & Min 15\% token&51.2&49.8&51.3&49.2&50.1&49.4&49.9&49.2&49.2&49.6&51.1\\
 & Min 25\% token&51.0&49.4&51.4&49.5&50.0&49.6&50.2&49.0&49.2&49.8&51.1\\
 \cline{1-2}\multirow{3}{*}{A\ref{as:exact_memorization}} & Mem 1&49.2&48.9&50.5&47.1&49.8&50.7&49.6&50.6&49.4&48.3&49.7\\
 & Mem 3&49.7&50.0&51.0&46.5&50.1&49.8&51.5&50.5&48.2&49.3&48.7\\
 & Mem 5&49.7&48.0&50.8&48.2&49.7&52.7&50.8&50.2&49.1&50.0&49.4\\
\cline{1-2} \multirow{3}{*}{A\ref{as:Generation_Variation}} & Entropy 5&51.9&49.2&52.4&48.9&50.3&48.0&49.4&51.9&48.6&49.0&50.4\\
 & Entropy 10&52.2&49.4&52.3&49.3&50.4&48.2&48.7&52.1&48.6&49.0&50.6\\
 & Entropy 25&52.1&49.5&50.9&49.5&50.7&48.5&48.1&51.0&48.1&49.6&50.9\\
\hline\multirow{2}{*}{PPL} & Seen&3.0$\pm$5.6&3.9$\pm$1.4&5.6$\pm$2.4&5.6$\pm$2.1&7.8$\pm$10.6&8.7$\pm$4.4&9.5$\pm$3.4&10.8$\pm$9.2&11.0$\pm$13.2&12.1$\pm$5.9&13.9$\pm$11.8\\
 & Unseen&3.0$\pm$6.2&4.0$\pm$3.0&5.7$\pm$2.1&5.6$\pm$2.2&8.0$\pm$10.4&8.6$\pm$4.3&9.6$\pm$3.6&10.6$\pm$8.2&10.8$\pm$13.2&11.8$\pm$5.5&13.9$\pm$10.5\\

    \hline
    \end{tabular}
    }
    \caption{Average contamination detection AUC for the Pythia-6.9b model, under different PILE domains. `PPL' represents the average perplexity $\pm$ STD, where instances are truncated by the model max length of 2048 tokens. The columns (domains) are sorted by the average PPL among the seen instances.
    }
    \label{tab:results_6.9b}
    \vspace{-10pt}
    \end{table*}
    

==> archive/tables/overall_70m.tex <==

\begin{table*}[h]
\centering
\resizebox{0.98\textwidth}{!}{
\begin{tabular}{llccccccccccc}
\hline
\multicolumn{2}{l}{\textbf{Assumptions \& Metric}} & \textbf{Github} & \textbf{\begin{tabular}[c]{@{}c@{}}Free-\\ Law\end{tabular}} & \textbf{ArXiv} & \textbf{\begin{tabular}[c]{@{}c@{}}PubMed\\ Central\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Enron\\ Emails\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}PubMed\\ Abstracts\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Open-\\ Subtitles\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}OpenWeb-\\ Text2\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Youtube-\\ Subtitles\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Hacker-\\ News\end{tabular}} & \textbf{Pile-CC} \\\hline
\multirow{6}{*}{A\ref{as:prob_absolute}}  & PPL\_50&49.7&48.9&50.7&49.4&49.6&49.7&47.9&50.3&50.8&48.4&49.8\\
 & PPL\_100&50.8&49.4&51.1&50.1&50.5&48.8&48.1&48.9&50.3&47.3&50.4\\
 & PPL\_200&51.1&49.4&50.9&50.2&51.4&49.9&47.8&48.5&49.5&50.7&52.1\\
 & Min 5\% token&51.5&49.8&51.3&48.5&50.0&48.5&49.8&49.7&49.0&47.8&50.9\\
 & Min 15\% token&51.2&49.8&51.3&49.2&50.1&49.4&49.9&49.2&49.2&49.6&51.1\\
 & Min 25\% token&51.0&49.4&51.4&49.5&50.0&49.6&50.2&49.0&49.2&49.8&51.1\\
 \cline{1-2}\multirow{3}{*}{A\ref{as:exact_memorization}} & Mem 1&49.2&48.9&50.5&47.1&49.8&50.7&49.6&50.6&49.4&48.3&49.7\\
 & Mem 3&49.7&50.0&51.0&46.5&50.1&49.8&51.5&50.5&48.2&49.3&48.7\\
 & Mem 5&49.7&48.0&50.8&48.2&49.7&52.7&50.8&50.2&49.1&50.0&49.4\\
\cline{1-2} \multirow{3}{*}{A\ref{as:Generation_Variation}} & Entropy 5&51.9&49.2&52.4&48.9&50.3&48.0&49.4&51.9&48.6&49.0&50.4\\
 & Entropy 10&52.2&49.4&52.3&49.3&50.4&48.2&48.7&52.1&48.6&49.0&50.6\\
 & Entropy 25&52.1&49.5&50.9&49.5&50.7&48.5&48.1&51.0&48.1&49.6&50.9\\
\hline\multirow{2}{*}{PPL} & Seen&10.8$\pm$25.2&13.1$\pm$5.4&17.2$\pm$9.2&16.0$\pm$7.6&137.4$\pm$1682.7&29.1$\pm$15.6&26.2$\pm$7.5&43.3$\pm$49.5&37.3$\pm$46.5&42.0$\pm$24.1&50.0$\pm$44.6\\
 & Unseen&10.5$\pm$19.6&13.7$\pm$13.4&18.6$\pm$34.0&15.8$\pm$7.4&38.9$\pm$44.7&29.2$\pm$22.7&26.1$\pm$8.7&41.7$\pm$31.5&36.9$\pm$37.1&40.8$\pm$21.0&49.8$\pm$36.1\\

    \hline
    \end{tabular}
    }
    \caption{Average contamination detection AUC for the \textbf{Pythia-70m} model, under different PILE domains. `PPL' represents the average perplexity $\pm$ STD, where instances are truncated by the model max length of 2048 tokens.
    }
    \label{tab:results_70m}
    \end{table*}
    

==> tables/GitHub.tex <==
\begin{table}[h]
\centering
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{lccccccc}
\hline
\multicolumn{1}{l}{\multirow{2}{*}{\textbf{Metric}}} & \multicolumn{7}{c}{\textbf{Model Size}} \\ \cline{2-8} 
\multicolumn{1}{c}{} & \textbf{70m} & \textbf{160m} & \textbf{410m} & \textbf{1b} & \textbf{1.4b} & \textbf{2.8b} & \textbf{6.9b} \\ \hline
ppl\_100 & 50.0 & 51.6 & 49.5 & 51.1 & 51.1 & 50.8 & 50.7 \\
ppl\_200 & 51.3 & 52.7 & 51.0 & 51.7 & 51.6 & 51.2 & 51.2 \\
ppl\_500 & 51.5 & 53.1 & 51.6 & 51.7 & 51.6 & 51.2 & 51.5 \\
Min 5\% token & 52.6 & 51.1 & 52.0 & 50.9 & 50.8 & 51.0 & 50.9 \\
Min 15\% token & 51.9 & 50.4 & 51.4 & 50.0 & 49.9 & 49.9 & 50.0 \\
Min 25\% token & 51.9 & 50.3 & 51.4 & 49.9 & 49.8 & 49.7 & 49.8 \\
Mem. 1 & 49.4 & 49.6 & 48.8 & 49.9 & 49.6 & 49.3 & 49.7 \\
Mem. 3 & 49.4 & 51.1 & 49.9 & 51.0 & 51.0 & 50.5 & 50.6 \\
Mem. 5 & 48.7 & 50.1 & 49.4 & 51.5 & 51.3 & 51.2 & 50.9 \\
Entropy 5 & 49.8 & 49.2 & 49.4 & 48.7 & 48.2 & 48.5 & 48.2 \\
Entropy 10 & 49.9 & 49.3 & 50.0 & 49.1 & 48.8 & 48.6 & 48.3 \\
Entropy 25 & 50.2 & 49.3 & 50.2 & 49.1 & 49.2 & 48.9 & 48.6 \\ \hline
Average & 50.6 & 50.7 & 50.4 & 50.4 & 50.2 & 50.1 & 50.0 \\ \hline
\end{tabular}
}
\caption{Detection AUC of each method, across different Pythia models, within the GitHub domain.}
\label{tab:github}
\end{table}

==> tables/OLMo-2-1124-7B.tex <==

\begin{table*}[h]
\centering
\resizebox{0.98\textwidth}{!}{
\begin{tabular}{llccccccccccc}
\hline
\multicolumn{2}{l}{\textbf{Assumptions \& Metric}} 
& \textbf{cpp}& \textbf{python}& \textbf{Github-Lean}& \textbf{julia}& \textbf{tex}& \textbf{Github-Isabelle}& \textbf{fortran}& \textbf{Github-Coq}& \textbf{r}\\\hline
\multirow{6}{*}{A\ref{as:prob_absolute}}  & PPL\_50& 51.1 & 51.7 & 49.9 & 50.2 & 49.4 & 50.9 & 50.3 & 49.1 & 49.5 
 & PPL\_100& 51.4 & 51.6 & 52.0 & 51.3 & 50.4 & 51.7 & 50.6 & 49.1 & 51.4 
 & PPL\_200& 51.8 & 50.8 & 51.2 & 51.6 & 50.0 & 50.8 & 51.1 & 49.0 & 53.0 
 & Min 5\% token& 50.1 & 51.1 & 49.0 & 52.0 & 49.4 & 51.2 & 48.1 & 49.4 & 50.9 
 & Min 15\% token& 50.2 & 50.4 & 50.7 & 51.2 & 48.6 & 50.4 & 48.1 & 49.0 & 51.5 
 & Min 25\% token& 50.3 & 49.8 & 51.3 & 51.0 & 48.7 & 49.9 & 48.2 & 48.9 & 52.4 
 \cline{1-2}\multirow{3}{*}{A\ref{as:exact_memorization}} & Mem 1& 50.9 & 48.6 & 46.4 & 49.8 & 48.7 & 50.7 & 48.8 & 51.3 & 50.6 
 & Mem 3& 50.7 & 50.0 & 51.9 & 49.7 & 48.8 & 55.5 & 50.7 & 50.4 & 51.2 
 & Mem 5& 51.6 & 48.9 & 52.9 & 49.2 & 48.6 & 54.9 & 50.7 & 49.6 & 51.4 
\cline{1-2} \multirow{3}{*}{A\ref{as:Generation_Variation}} & Entropy 5& 50.2 & 49.4 & 51.7 & 51.3 & 48.8 & 49.0 & 48.8 & 48.9 & 54.1 
 & Entropy 10& 50.2 & 49.4 & 51.8 & 51.3 & 48.8 & 48.9 & 48.8 & 49.0 & 53.6 
 & Entropy 25& 50.3 & 49.5 & 51.8 & 51.2 & 48.8 & 49.0 & 48.8 & 49.0 & 53.5 \\\hline
\multicolumn{2}{l}{\textbf{Average AUC}}& 50.6 & 50.0 & 51.0 & 50.9 & 49.0 & 50.7 & 49.3 & 49.3 & 52.2 
\hline\multirow{2}{*}{PPL\_200} & Seen& 4.3$\pm$2.6 & 6.7$\pm$3.9 & 6.9$\pm$3.4 & 8.3$\pm$5.0 & 8.3$\pm$5.1 & 8.7$\pm$5.4 & 9.5$\pm$6.8 & 10.4$\pm$8.3 & 10.5$\pm$7.0 
 & Unseen& 4.6$\pm$3.0 & 6.8$\pm$4.1 & 6.9$\pm$3.0 & 8.6$\pm$5.6 & 8.7$\pm$6.3 & 9.2$\pm$6.5 & 9.9$\pm$7.6 & 9.9$\pm$7.2 & 10.5$\pm$5.6 

\hline
\end{tabular}
}
\caption{Average contamination detection AUC for the OLMo-2-1124-7B model,  under different domains within
the Algebraic Stack dataset. `PPL\_200' represents the average perplexity $\pm$ STD, from the first 200 tokens within every instance.  The color {\color[HTML]{38761D} green} represents AUCs higher than 60.
}
\label{tab:results_OLMo-2-1124-7B}
\end{table*}


==> tables/PILE-cc.tex <==
\begin{table}[h]
\centering
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{lccccccc}
\hline
\multicolumn{1}{l}{\multirow{2}{*}{\textbf{Metric}}} & \multicolumn{7}{c}{\textbf{Model Size}} \\ \cline{2-8} 
\multicolumn{1}{c}{} & \textbf{70m} & \textbf{160m} & \textbf{410m} & \textbf{1b} & \textbf{1.4b} & \textbf{2.8b} & \textbf{6.9b} \\ \hline
PPL\_100 & 93.0 & 92.4 & 93.7 & 94.1 & 94.2 & 94.5 & 94.8 \\
PPL\_200 & 95.3 & 95.1 & 96.2 & 96.4 & 96.5 & 96.7 & 96.9 \\
PPL\_500 & 97.0 & 97.0 & 97.7 & 97.8 & 97.8 & 97.9 & 97.9 \\
Min 5\% token & 85.4 & 87.7 & 89.7 & 90.6 & 90.4 & 90.8 & 91.1 \\
Min 15\% token & 88.1 & 89.6 & 90.7 & 91.4 & 91.3 & 91.7 & 92.2 \\
Min 25\% token & 89.4 & 90.4 & 91.4 & 92.1 & 92.1 & 92.4 & 92.9 \\
Mem. 1 & 85.8 & 89.3 & 86.4 & 86.4 & 87.0 & 86.7 & 85.9 \\
Mem. 3 & 92.0 & 92.7 & 91.0 & 91.5 & 90.8 & 91.3 & 90.2 \\
Mem. 5 & 95.0 & 95.0 & 94.3 & 94.1 & 93.0 & 93.6 & 92.4 \\
Entropy 5 & 75.2 & 77.9 & 78.9 & 81.0 & 82.0 & 82.2 & 82.0 \\
Entropy 10 & 75.4 & 77.8 & 78.8 & 80.7 & 81.7 & 81.8 & 82.1 \\
Entropy 25 & 75.4 & 77.2 & 78.1 & 79.5 & 80.2 & 80.5 & 80.9 \\ \hline
Average & 87.3 & 88.5 & 88.9 & 89.6 & 89.8 & 90.0 & 89.9 \\ \hline
\end{tabular}
}
\caption{Detection AUC of each method, across different Pythia models, within the Pile-CC domain.}
\label{tab:pile}
\end{table}

==> tables/overall_zephyr_7b_beta.tex <==

\begin{table*}[h]
\centering
\resizebox{0.98\textwidth}{!}{
\begin{tabular}{llccccccccccc}
\hline
\multicolumn{2}{l}{\textbf{Assumptions \& Metric}} 
& \textbf{UltraChatl}\\\hline
\multirow{6}{*}{A\ref{as:prob_absolute}}  & PPL\_50& 55.3 \\ 
 & PPL\_100& 59.1 \\ 
 & PPL\_200& {\color[HTML]{38761D} \textbf{60.1}} \\ 
 & Min 5\% token& {\color[HTML]{38761D} \textbf{63.6}} \\ 
 & Min 15\% token& {\color[HTML]{38761D} \textbf{63.0}} \\ 
 & Min 25\% token& {\color[HTML]{38761D} \textbf{61.5}} \\ 
 \cline{1-2}\multirow{3}{*}{A\ref{as:exact_memorization}} & Mem 5& 52.2 \\ 
 & Mem 15& 53.1 \\ 
 & Mem 25& 53.1 \\ 
\cline{1-2} \multirow{3}{*}{A\ref{as:Generation_Variation}} & Entropy 5& 54.3 \\ 
 & Entropy 15& 54.1 \\ 
 & Entropy 25& 54.0 \\\hline
\multicolumn{2}{l}{\textbf{Average AUC}}& 55.9 \\ 
\hline\multirow{2}{*}{PPL\_200} & Seen& 5.3$\pm$4.6 \\ 
 & Unseen& 6.2$\pm$4.1 \\ 

\hline
\end{tabular}
}
\caption{Average contamination detection AUC for the \textbf{zephyr-7b-beta} model,  under different domains within
the Algebraic Stack dataset. `PPL\_200' represents the average perplexity $\pm$ STD, from the first 200 tokens within every instance.  The color {\color[HTML]{38761D} green} represents AUCs higher than 60.
}
\label{tab:results_zephyr-7b-beta}
\end{table*}


==> tables/summary_indirect_task.tex <==
\begin{table}[h]
\centering

\resizebox{0.45\textwidth}{!}{
\begin{tabular}{ll}
\hline
\textbf{\begin{tabular}[c]{@{}l@{}}Contami-\\ nation\end{tabular}} & \textbf{Detection Research} \\ \hline
\begin{tabular}[c]{@{}l@{}}Indirect\\ Data\end{tabular}          &  \begin{tabular}[c]{@{}l@{}} \citet{dong2024generalization}, \citet{yang2023rethinking},\\\citet{balloccu2024leak} \end{tabular}   \\ \hline
Task                   &   \begin{tabular}[c]{@{}l@{}} \citet{li2024task}, \citet{ranaldi2024investigating},\\ \citet{aiyappa-etal-2023-trust}, \citet{cao2024concerned}\end{tabular}     \\ \hline
\end{tabular}
}
\caption{Existing detection approaches for indirect data contamination and task contamination.}
\label{tab:indirect_task}
\end{table}

% Indirect & - & - & \citet{dong2024generalization}, \citet{yang2023rethinking} &  \\ \hline

% Task & \begin{tabular}[c]{@{}l@{}}Performance \\ Change \end{tabular} & \begin{tabular}[c]{@{}l@{}}Similar Tasks \\ (Assumption \ref{as:same_difficulty})\end{tabular} & \begin{tabular}[c]{@{}l@{}} \citet{li2024task}, \citet{ranaldi2024investigating},\\ \citet{aiyappa-etal-2023-trust}, \citet{cao2024concerned}\end{tabular} &  \\ \hline

==> tables/summary_old.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}



\begin{table*}[h]
\centering
\resizebox{0.99\textwidth}{!}{

\begin{tabular}{lllll}
\hline
\textbf{\begin{tabular}[c]{@{}l@{}}Contami-\\ nation\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Detection\\ Approach\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Assumptions / \\ Requirements\end{tabular}} & \textbf{Detection Research} & \textbf{\begin{tabular}[c]{@{}l@{}}Critiques on\\ Those Approaches \end{tabular}} \\ \hline
 & \begin{tabular}[c]{@{}l@{}}Instance\\ Similarity\end{tabular} & \underline{\textcolor{orange}{Requirement}} \ref{condi:disclose} \& \ref{condi:accessible} & \begin{tabular}[c]{@{}l@{}}\citet{dodge2021documenting}, \citet{elangovan2021memorization}, \\ \citet{li2023open}, \citet{riddell2024quantifying}, \\ \citet{deng2024investigating}, \citet{yang2023rethinking}, \\ \citet{piktus2023roots}, \citet{lee2022deduplicating},\\ \citet{NEURIPS2023_3112ee70}\end{tabular} &  \\ \cline{2-5} 
 &  & \begin{tabular}[c]{@{}l@{}}Ref Prob. by Instance\\ (Assumption \ref{as:prob_reference_sent})\end{tabular} &  \begin{tabular}[c]{@{}l@{}}\citet{mattern2023membership}, \citet{maini2024llm} \\ \citet{oren2024proving} \end{tabular}& \citet{maini2024llm} \\ \cline{3-5} %
 &  & \begin{tabular}[c]{@{}l@{}}Ref Prob. by LM\\ (Assumption \ref{as:prob_normalized_sent})\end{tabular} & \begin{tabular}[c]{@{}l@{}}\citet{carlini2021extracting},  \citet{maini2024llm}, \\ \citet{mireshghallah-etal-2022-quantifying},\\ \citet{zanella2020analyzing}\end{tabular} & {\begin{tabular}[c]{@{}l@{}}\citet{dekoninck2024evading},\\ \citet{duan2024membership}, \\ \citet{cao2024concerned}\end{tabular}} \\ \cline{3-5} 
 &  & \begin{tabular}[c]{@{}l@{}}\underline{\textcolor{orange}{Absolute Prob}}\\ (Assumption \ref{as:prob_absolute})\end{tabular} & \begin{tabular}[c]{@{}l@{}}\citet{10.1145/3292500.3330885}, \\ \citet{shi2023detecting}, \citet{li2023estimating}, \\ \citet{maini2024llm},\citet{wei-etal-2024-proving},  \\ \citet{srivastava2023beyond}\end{tabular} & \begin{tabular}[c]{@{}l@{}}\citet{dekoninck2024evading}, \\ \citet{duan2024membership}, \\ \citet{maini2024llm}, \\ \citet{cao2024concerned}\end{tabular} \\ \cline{3-5} 
 & \multirow{-10}{*}{\begin{tabular}[c]{@{}l@{}}Probability\\ Analysis\end{tabular}} & Other & \begin{tabular}[c]{@{}l@{}}\citet{jagannatha2021membership}, \citet{zhang2023counterfactual}\end{tabular} &  \\ \cline{2-5} 
 
 
 &  & \begin{tabular}[c]{@{}l@{}}\underline{\textcolor{orange}{Verbatim}} \\ \underline{\textcolor{orange}{Memorization}}\\ (Assumption \ref{as:exact_memorization})\end{tabular} & \begin{tabular}[c]{@{}l@{}}\citet{carliniquantifying}, \citet{kandpal2022deduplicating},\\ \citet{magar2022data}, \citet{duarte2024decop}, \\ \citet{Golchin2023quiz}\end{tabular} &  \\ \cline{3-5} 
 &  & \begin{tabular}[c]{@{}l@{}}Key Information \\ Generation\\ (Assumption \ref{as:key_memorization})\end{tabular} & \begin{tabular}[c]{@{}l@{}}\citet{deng2024investigating}, \citet{ranaldi2024investigating},\\ \citet{chang2023speak}, \citet{9152761},\\ \citet{carlini2021extracting}, \citet{236216},\\ \citet{tirumala2022memorization}, \citet{liu-etal-2024-evaluating},\\ \citet{golchintime},\\\citet{Golchin2023quiz}\end{tabular} & \citet{dekoninck2024evading} \\ \cline{3-5} 
 &  & \begin{tabular}[c]{@{}l@{}}\underline{\textcolor{orange}{Generation Variation}}\\ (Assumption \ref{as:Generation_Variation})\end{tabular} & \citet{dong2024generalization} &  \\ \cline{3-5} 
 &  & \begin{tabular}[c]{@{}l@{}}Metadata-based \\ Memorization\\ (Assumption \ref{as:meta_data})\end{tabular} & \begin{tabular}[c]{@{}l@{}}\citet{sainz2023chatgpt}\\ \citet{karamolegkou-etal-2023-copyright}\end{tabular} &  \\ \cline{3-5} 
\multirow{-30}{*}{Direct} & \multirow{-15}{*}{\begin{tabular}[c]{@{}l@{}}Instance\\ Generation \\ \& \\ Instance\\ Selection \\ \end{tabular}} & Other & \citet{schwarzschild2024rethinking} &  \\ \cline{2-5}
 & \begin{tabular}[c]{@{}l@{}}Answer\\ Memorization\end{tabular} & \begin{tabular}[c]{@{}l@{}}Instance Perturbation \\ (Assumption \ref{as:same_task})\end{tabular} & \begin{tabular}[c]{@{}l@{}} \citet{liu-etal-2024-evaluating}, \citet{mehrbakhsh-etal-2024-confounders}, \\ \citet{yim-etal-2024-err-human}, \citet{zong2023fool}, \\ \citet{razeghi2022impact}  \end{tabular} &  \\  \hline
Indirect & - & - & \citet{dong2024generalization}, \citet{yang2023rethinking} &  \\ \hline

Task & \begin{tabular}[c]{@{}l@{}}Performance \\ Change \end{tabular} & \begin{tabular}[c]{@{}l@{}}Similar Tasks \\ (Assumption \ref{as:same_difficulty})\end{tabular} & \begin{tabular}[c]{@{}l@{}} \citet{li2024task}, \citet{ranaldi2024investigating},\\ \citet{aiyappa-etal-2023-trust}, \citet{cao2024concerned}\end{tabular} &  \\ \hline

% \multirow{4}{*}{Task} & \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}Performance\\ Change\end{tabular}} & \begin{tabular}[c]{@{}l@{}}Same Task \\ (Assumption \ref{as:same_task})\end{tabular} & \begin{tabular}[c]{@{}l@{}} \citet{liu-etal-2024-evaluating}, \citet{mehrbakhsh-etal-2024-confounders}, \\ \citet{yim-etal-2024-err-human}, \citet{zong2023fool} \end{tabular} &  \\ \cline{3-5} 
 
% &  & \begin{tabular}[c]{@{}l@{}}Similar Tasks \\ (Assumption \ref{as:same_difficulty})\end{tabular} & \begin{tabular}[c]{@{}l@{}}\citet{li2024task}, \citet{ranaldi2024investigating},\\ \citet{aiyappa-etal-2023-trust}, \citet{cao2024concerned}, \\ \citet{razeghi2022impact}\end{tabular} &  \\ \hline%\cline{3-5} 

%\multirow{-5}{*}{Task} & Novel Tasks & \begin{tabular}[c]{@{}l@{}} Task Unseen \\ (Assumption \ref{as:task_unseen})\end{tabular} & \citet{li-etal-2024-challenging},  &  \\ \hline

\end{tabular}
}

\caption{Existing detection approaches for data contamination, their assumptions, and Critiques they received. Our investigation and case study show that the \textcolor{orange}{orange}, \underline{underlined} assumptions and requirements are not always satisfied.}
\label{tab:summmary_old}
\end{table*}

% needs to adjust the \multirow{-, for space in the contamination row.

% to change 
% \citet{
% }
% _
% \ref{

==> tables/zephyr-7b-beta.tex <==

\begin{table*}[h]
\centering
\resizebox{0.98\textwidth}{!}{
\begin{tabular}{llccccccccccc}
\hline
\multicolumn{2}{l}{\textbf{Assumptions \& Metric}} 
& \textbf{UltraChatl}\\\hline
\multirow{6}{*}{A\ref{as:prob_absolute}}  & PPL\_50& 55.3 
 & PPL\_100& 59.1 
 & PPL\_200& {\color[HTML]{38761D} \textbf{60.1}} 
 & Min 5\% token& {\color[HTML]{38761D} \textbf{63.6}} 
 & Min 15\% token& {\color[HTML]{38761D} \textbf{63.0}} 
 & Min 25\% token& {\color[HTML]{38761D} \textbf{61.5}} 
 \cline{1-2}\multirow{3}{*}{A\ref{as:exact_memorization}} & Mem 1& 51.5 
 & Mem 3& 52.6 
 & Mem 5& 51.9 
\cline{1-2} \multirow{3}{*}{A\ref{as:Generation_Variation}} & Entropy 5& 54.3 
 & Entropy 10& 54.2 
 & Entropy 25& 54.0 \\\hline
\multicolumn{2}{l}{\textbf{Average AUC}}& 56.7 
\hline\multirow{2}{*}{PPL\_200} & Seen& 5.3$\pm$4.6 
 & Unseen& 6.2$\pm$4.1 

\hline
\end{tabular}
}
\caption{Average contamination detection AUC for the zephyr-7b-beta model,  under different domains within
the Algebraic Stack dataset. `PPL\_200' represents the average perplexity $\pm$ STD, from the first 200 tokens within every instance.  The color {\color[HTML]{38761D} green} represents AUCs higher than 60.
}
\label{tab:results_zephyr-7b-beta}
\end{table*}

